More on $G$-flux and General Hodge Cycles on the Fermat Sextic

We study M-Theory solutions with $G$-flux on the Fermat sextic Calabi-Yau fourfold, focussing on the relationship between the number of stabilized complex structure moduli and the tadpole contribution of the flux. We use two alternative approaches to define the fluxes: algebraic cycles and (appropriately quantized) Griffiths residues. In both cases, we collect evidence for the non-existence of solutions which stabilize all moduli and stay within the tadpole bound

==> text <==
add reference taizan


CM type in IIB, number fields   

\bibitem{Kanno:2017nub}
K.~Kanno and T.~Watari,
%``Revisiting arithmetic solutions to the $W=0$ condition,''
Phys. Rev. D \textbf{96} (2017) no.10, 106001
doi:10.1103/PhysRevD.96.106001
[arXiv:1705.05110 [hep-th]].



\bibitem{Kanno:2020kxr}
K.~Kanno and T.~Watari,
%``W = 0 Complex Structure Moduli Stabilization on CM-type K3 $\times $ K3 Orbifolds: Arithmetic, Geometry and Particle Physics,''
Commun. Math. Phys. \textbf{398} (2023) no.2, 703-756
doi:10.1007/s00220-022-04533-4
[arXiv:2012.01111 [hep-th]].
